A robust collision source method for rank adaptive dynamical low-rank approximation in radiation therapy

Deterministic models for radiation transport describe the density of radiation particles moving through a background material. In radiation therapy applications, the phase space of this density is composed of energy, spatial position and direction of flight. The resulting six-dimensional phase space prohibits fine numerical discretizations, which are essential for the construction of accurate and reliable treatment plans. In this work, we tackle the high dimensional phase space through a dynamical low-rank approximation of the particle density. Dynamical low-rank approximation (DLRA) evolves the solution on a low-rank manifold in time. Interpreting the energy variable as a pseudo-time lets us employ the DLRA framework to represent the solution of the radiation transport equation on a low-rank manifold for every energy. Stiff scattering terms are treated through an efficient implicit energy discretization and a rank adaptive integrator is chosen to dynamically adapt the rank in energy. To facilitate the use of boundary conditions and reduce the overall rank, the radiation transport equation is split into collided and uncollided particles through a collision source method. Uncollided particles are described by a directed quadrature set guaranteeing low computational costs, whereas collided particles are represented by a low-rank solution. It can be shown that the presented method is L$^2$-stable under a time step restriction which does not depend on stiff scattering terms. Moreover, the implicit treatment of scattering does not require numerical inversions of matrices. Numerical results for radiation therapy configurations as well as the line source benchmark underline the efficiency of the proposed method.

==> ideas.tex <==

----------------------------------------------------------------------------------------------------------

The efficient $L$-step projector--splitting computation gives
\begin{align*}
    \mathbf{S}^1 = \mathbf{S}^0+\Delta t \mathbf{X}^{1,T}\mathbf{u}^{n+1}\bm{\Sigma} (\mathbf{I}+\Delta t\Sigma_t \mathbf{I}-\Delta t \bm{\Sigma} )^{-1}\mathbf{W}^1
\end{align*}
Taking norms gives
\begin{align*}
    \Vert\mathbf{S}^1\Vert_F \leq& \Vert\mathbf{S}^0\Vert_F+\Delta t \Vert\mathbf{u}^{n+1}\Vert_F \Vert \bm{\Sigma} (\mathbf{I}+\Delta t\Sigma_t \mathbf{I}-\Delta t \bm{\Sigma} )^{-1}\Vert\\
    =&\Vert\mathbf{S}^0\Vert_F+ \max_k \frac{\Delta t\sigma_k}{1+\Delta t\sigma_t-\Delta t\sigma_k} \cdot\Vert\mathbf{u}^{n+1}\Vert_F 
\end{align*}
Add $\Vert\mathbf{u}^{n+1}\Vert_F$ on both sides to get
\begin{align*}
    \Vert\mathbf{S}^1\Vert_F + \Vert\mathbf{u}^{n+1}\Vert_F \leq& \Vert\mathbf{S}^0\Vert_F+ \max_k \frac{1+\Delta t\sigma_t}{1+\Delta t\sigma_t-\Delta t\sigma_k} \cdot\Vert\mathbf{u}^{n+1}\Vert_F \\
    =& \Vert\mathbf{S}^0\Vert_F+ \max_k \frac{1}{1+\Delta t\sigma_t-\Delta t\sigma_k} \cdot\Vert\mathbf{u}^{n}\Vert_F
\end{align*}

----------------------------------------------------------------------------------------------------------

\begin{align*}
    \mathbf{\widehat S}^1 =& \ \mathbf{\widetilde S}^0 + \Delta t\mathbf{X}^{1,T}\bm u^{n+1}\mathbf{W}^1\bm{\widehat \Sigma}^1(\mathbf I+\sigma_t\Delta t\mathbf I - \Delta t\bm{\widehat \Sigma}^1)^{-1}
\end{align*}


\begin{align*}
    \mathbf{\widehat S}_{c}^1 =& \ \mathbf{\widetilde S}_{c}^0 + \Delta t\mathbf{X}_{c}^{1,T}\mathbf{X}_{L}^{1}\mathbf{S}_{L}^1\mathbf{W}_{L}^{1,T}\mathbf{\widetilde W}_{c}^1\mathbf{\widetilde W}_{c}^{1,T}\bm{\Sigma}(t_1)\mathbf{\widetilde W}_{c}^1,\\
    \mathbf{S}_c^{1} =& \ \mathbf{\widehat S}_{c}^1 (\mathbf I+\sigma_t\Delta t\mathbf I - \Delta t\mathbf{\widetilde W}_{c}^{1,T}\bm{\Sigma}(t_1)\mathbf{\widetilde W}_{c}^1)^{-1}
\end{align*}


\begin{align*}
    \mathbf{\widehat S}_{c}^1 =& \ \mathbf{\widetilde S}_{c}^0 + \Delta t\mathbf{X}_{c}^{1,T}\mathbf{X}_{L}^{1}\mathbf{S}_{L}^1\mathbf{W}_{L}^{1,T}\mathbf{\widetilde W}_{c}^1\bm{\widehat \Sigma},\\
    \mathbf{S}_c^{1} =& \ \mathbf{\widehat S}_{c}^1 (\mathbf I+\sigma_t\Delta t\mathbf I - \Delta t\bm{\widehat \Sigma})^{-1}
\end{align*}

\begin{align*}
    \mathbf{S}_c^{1} =& \ \mathbf{\widetilde S}_{c}^0(\mathbf I+\sigma_t\Delta t\mathbf I + \Delta t\bm{\widehat \Sigma})^{-1}\\
    &+ \Delta t\mathbf{X}_{c}^{1,T}\mathbf{X}_{L}^{1}\mathbf{S}_{L}^1\mathbf{W}_{L}^{1,T}\mathbf{\widetilde W}_{c}^1\bm{\widehat \Sigma}(\mathbf I+\sigma_t\Delta t\mathbf I - \Delta t\bm{\widehat \Sigma})^{-1}
\end{align*}
Define $\mathbf{\widehat S}_{L}^1:=\mathbf{X}_{c}^{1,T}\mathbf{X}_{L}^{1}\mathbf{S}_{L}^1\mathbf{W}_{L}^{1,T}\mathbf{\widetilde W}_{c}^1$
\begin{align*}
    \mathbf{S}_c^{1}+\mathbf{\widehat S}_{L}^1 =& \ \mathbf{\widetilde S}_{c}^0(\mathbf I+\sigma_t\Delta t\mathbf I + \Delta t\bm{\widehat \Sigma})^{-1}+ \left(\Delta t\mathbf{\widehat S}_{L}^1\bm{\widehat \Sigma}\right)(\mathbf I+\sigma_t\Delta t\mathbf I - \Delta t\bm{\widehat \Sigma})^{-1}+\mathbf{\widehat S}_{L}^1 \\
    =& \ \mathbf{\widetilde S}_{c}^0(\mathbf I+\sigma_t\Delta t\mathbf I + \Delta t\bm{\widehat \Sigma})^{-1}\\
    &+ \left(\mathbf{\widehat S}_{L}^1(\mathbf I+\sigma_t\Delta t\mathbf I - \Delta t\bm{\widehat \Sigma}) + \Delta t\mathbf{\widehat S}_{L}^1\bm{\widehat \Sigma}\right)(\mathbf I+\sigma_t\Delta t\mathbf I - \Delta t\bm{\widehat \Sigma})^{-1} \\
    =& \ \mathbf{\widetilde S}_{c}^0(\mathbf I+\sigma_t\Delta t\mathbf I + \Delta t\bm{\widehat \Sigma})^{-1}\\
    &+ \mathbf{\widehat S}_{L}^1(\mathbf I+\sigma_t\Delta t\mathbf I)(\mathbf I+\sigma_t\Delta t\mathbf I - \Delta t\bm{\widehat \Sigma})^{-1} \\
\end{align*}

----------------------------------------------------------------------------------------------------------
\begin{align*}
    \mathbf{\widetilde L}_{c}^1 =& \ \mathbf{\widehat S}_{c}^1\mathbf{\widetilde W}_{c}^{1,T} (\mathbf I+\sigma_t\Delta t\mathbf I + \Delta t\bm{\Sigma})^{-1}\;.
\end{align*}

\begin{align*}
    \mathbf{X}_c^1\mathbf{S}_{c}^1\mathbf{W}_{c}^{1,T} =& \ \left(\mathbf{X}_c^1\mathbf{\widetilde S}_{c}^0\mathbf{\widetilde W}_{c}^{1,T} + \Delta t\mathbf{X}_c^1\mathbf{X}_{c}^{1,T}\mathbf{X}_{L}^{1}\mathbf{S}_{L}^1\mathbf{W}_{L}^{1,T}\mathbf{\widetilde W}_{c}^1\mathbf{\widetilde W}_{c}^{1,T}\bm{\Sigma}(t_1)\mathbf{\widetilde W}_{c}^1\mathbf{\widetilde W}_{c}^{1,T}\right) (\mathbf I+\sigma_t\Delta t\mathbf I - \Delta t\bm{\Sigma})^{-1}\;.
\end{align*}

\begin{align*}
    \Vert\mathbf{X}_c^1\mathbf{S}_{c}^1\mathbf{W}_{c}^{1,T}\Vert_F\bm I \leq& \ \left(\Vert\mathbf{X}_c^1\mathbf{\widetilde S}_{c}^0\mathbf{\widetilde W}_{c}^{1,T}\Vert_F + \Vert \Delta t\mathbf{X}_c^1\mathbf{X}_{c}^{1,T}\mathbf{X}_{L}^{1}\mathbf{S}_{L}^1\mathbf{W}_{L}^{1,T}\mathbf{\widetilde W}_{c}^1\mathbf{\widetilde W}_{c}^{1,T}\bm{\Sigma}(t_1)\mathbf{\widetilde W}_{c}^1\mathbf{\widetilde W}_{c}^{1,T}\Vert_F\right)(\mathbf I+\sigma_t\Delta t\mathbf I - \Delta t\bm{\Sigma})^{-1}\;
\end{align*}

\begin{align*}
    &\Vert\mathbf{X}_c^1\mathbf{S}_{c}^1\mathbf{W}_{c}^{1,T}\Vert_F\bm I+\Vert\mathbf{X}_c^1\mathbf{X}_c^{1,T}\mathbf{X}_L^1\mathbf{S}_{L}^1\mathbf{W}_{L}^{1,T}\Vert_F\bm I \leq \ \Vert\mathbf{X}_c^1\mathbf{\widetilde S}_{c}^0\mathbf{\widetilde W}_{c}^{1,T}\Vert_F(\mathbf I+\sigma_t\Delta t\mathbf I - \Delta t\bm{\Sigma})^{-1}\\
    &+ \Vert \Delta t\mathbf{X}_c^1\mathbf{X}_{c}^{1,T}\mathbf{X}_{L}^{1}\mathbf{S}_{L}^1\mathbf{W}_{L}^{1,T}\mathbf{\widetilde W}_{c}^1\mathbf{\widetilde W}_{c}^{1,T}\bm{\Sigma}(t_1)\mathbf{\widetilde W}_{c}^1\mathbf{\widetilde W}_{c}^{1,T}\Vert_F(\mathbf I+\sigma_t\Delta t\mathbf I - \Delta t\bm{\Sigma})^{-1}+\Vert\mathbf{X}_c^1\mathbf{S}_{L}^1\mathbf{W}_{c}^{1,T}\Vert_F\bm I\;
\end{align*}

$||x|-|y||\leq|x-y|$
Plug this in to get single expression

\end{proof}

Now, we wish to determine the effect of scattering. With $\bm{\widehat u} := \bm{\psi}^{n+1}\bm M$ we have
\begin{align}
    \bm u^{n+1}(\bm I +\Delta t\sigma_t\bm I-\Delta t\bm\Sigma) =& \bm u^{n} + \Delta t\bm{\widehat u}^{n+1}\bm\Sigma\\
    \bm{\widehat u}^{n+1}(\bm I +\Delta t\sigma_t\bm I) =& \bm{\widehat u}^{n}
\end{align}

\begin{align}
    \bm u^{n+1}+\bm{\widehat u}^{n+1} = \bm u^{n}(\bm I +\Delta t\sigma_t\bm I-\Delta t\bm\Sigma)^{-1} + \Delta t\bm{\widehat u}^{n}(\bm I +\Delta t\sigma_t\bm I)^{-1}\bm\Sigma(\bm I +\Delta t\sigma_t\bm I-\Delta t\bm\Sigma)^{-1}+\bm{\widehat u}^{n}(\bm I +\Delta t\sigma_t\bm I)^{-1}
\end{align}
Let us pick a fixed moment order $i$:
\begin{align}
    \bm u^{n+1}_i+\bm{\widehat u}^{n+1}_i =& \ \frac{1}{1+\Delta t(\sigma_t-\sigma_i)}\bm u^{n}_i + \frac{\Delta t\sigma_i}{1+\Delta t(\sigma_t-\sigma_i)}\frac{1}{1+\Delta t\sigma_t}\bm{\widehat u}^{n}_i+\frac{1}{1+\Delta t\sigma_t}\bm{\widehat u}^{n}_i\\
    =& \ \frac{1}{1+\Delta t(\sigma_t-\sigma_i)}\left(\bm u^{n}_i + \frac{\Delta t\sigma_i}{1+\Delta t\sigma_t}\bm{\widehat u}^{n}_i+\frac{1+\Delta t(\sigma_t-\sigma_i)}{1+\Delta t\sigma_t}\bm{\widehat u}^{n}_i\right)\\
    =&\frac{1}{1+\Delta t(\sigma_t-\sigma_i)}\left(\bm u^{n}_i+\bm{\widehat u}^{n}_i\right)
\end{align}
Now for DLRA, the $S$-step is either
\begin{align*}
    \bm S^{n+1} =&\ \bm S^{n}\bm{W}^{n+1,T}(\bm I +\Delta t\sigma_t\bm I-\Delta t\bm\Sigma)^{-1}\bm{W}^{n+1} + \Delta t\bm{X}^{n+1,T}\bm{\widehat u}^{n+1}\bm\Sigma(\bm I +\Delta t\sigma_t\bm I-\Delta t\bm\Sigma)^{-1}\bm{W}^{n+1}\\
\bm{\widehat u}^{n+1} =&\ \bm{\widehat u}^{n}(\bm I +\Delta t\sigma_t\bm I)^{-1}
\end{align*}
or (if we are strict and accurate)
\begin{align}\label{eq:S1}
    \bm S^{n+1} =& \bm S^{n}-\Delta t\sigma_t\bm S^{n+1}+\Delta t\bm S^{n+1}\bm{W}^{n+1,T}\bm\Sigma\bm{W}^{n+1} + \Delta t\bm{X}^{n+1,T}\bm{\widehat u}^{n+1}\bm\Sigma\bm{W}^{n+1},\\
\bm{\widehat u}^{n+1} =& \bm{\widehat u}^{n}(\bm I +\Delta t\sigma_t\bm I)^{-1},
\end{align}
hence what we compute is 
\begin{align*}
    \bm S^{n+1} =& \left(\bm S^{n} + \Delta t\bm{X}^{n+1,T}\bm{\widehat u}^{n+1}\bm\Sigma\bm{W}^{n+1}\right)\left(\bm I+\Delta t\sigma_t-\Delta t\bm{W}^{n+1,T}\bm\Sigma\bm{W}^{n+1}\right)^{-1},\\
\bm{\widehat u}^{n+1} =& \bm{\widehat u}^{n}(\bm I +\Delta t\sigma_t\bm I)^{-1}.
\end{align*}
We define $\bm{\widehat \Sigma}:= \bm{W}^{n+1,T}\bm\Sigma\bm{W}^{n+1}$ and add $\bm{X}^{n+1,T}\bm{\widehat u}^{n+1}\bm{W}^{n+1}$ to get for $\bm S_{full}^{n+1} :=\bm S^{n+1} + \bm{X}^{n+1,T}\bm{\widehat u}^{n+1}\bm{W}^{n+1}$
\begin{align*}
\bm S_{full}^{n+1} =& \left(\bm S^{n} + \Delta t\bm{X}^{n+1,T}\bm{\widehat u}^{n+1}\bm\Sigma\bm{W}^{n+1}\right)\left(\bm I+\Delta t\sigma_t\bm I-\Delta t\bm{\widehat \Sigma}\right)^{-1}+ \bm{X}^{n+1,T}\bm{\widehat u}^{n+1}\bm{W}^{n+1}\\
=& \left(\bm S^{n} + \Delta t\bm{X}^{n+1,T}\bm{\widehat u}^{n+1}\bm\Sigma\bm{W}^{n+1}+ \bm{X}^{n+1,T}\bm{\widehat u}^{n+1}\bm{W}^{n+1}\left(\bm I+\Delta t\sigma_t-\Delta t\bm{\widehat \Sigma}\right)\right)\left(\bm I+\Delta t\sigma_t-\Delta t\bm{\widehat \Sigma}\right)^{-1}\\
=& \left(\bm S^{n} + \Delta t\bm{X}^{n+1,T}\bm{\widehat u}^{n+1}\left(\bm\Sigma +\frac1{\Delta t}\bm I+\sigma_t\bm I -\bm{W}^{n+1}\bm{\widehat \Sigma}\bm{W}^{n+1,T} \right)\bm{W}^{n+1}\right)\left(\bm I+\Delta t\sigma_t-\Delta t\bm{\widehat \Sigma}\right)^{-1}\\
=& \bm S^{n}\left(\bm I+\Delta t\sigma_t-\Delta t\bm{\widehat \Sigma}\right)^{-1}\\ 
&+ \Delta t\bm{X}^{n+1,T}\bm{\widehat u}^{n+1}\left(\bm\Sigma +\frac1{\Delta t}\bm I+\sigma_t\bm I -\bm{W}^{n+1}\bm{\widehat \Sigma}\bm{W}^{n+1,T} \right)\bm{W}^{n+1}\left(\bm I+\Delta t\sigma_t-\Delta t\bm{\widehat \Sigma}\right)^{-1}\\
=& \bm S^{n}\left(\bm I+\Delta t\sigma_t-\Delta t\bm{\widehat \Sigma}\right)^{-1}\\ 
&+ \frac{\Delta t}{1+\Delta t \sigma_t}\bm{X}^{n+1,T}\bm{\widehat u}^{n}\left(\bm\Sigma +\frac1{\Delta t}\bm I+\sigma_t\bm I -\bm{W}^{n+1}\bm{\widehat \Sigma}\bm{W}^{n+1,T} \right)\bm{W}^{n+1}\left(\bm I+\Delta t\sigma_t-\Delta t\bm{\widehat \Sigma}\right)^{-1}\\
=& (\bm S^{n} +\bm{X}^{n+1,T}\bm{\widehat u}^{n}\bm{W}^{n+1})\left(\bm I+\Delta t\sigma_t-\Delta t\bm{\widehat \Sigma}\right)^{-1}\\ 
&+ \frac{\Delta t}{1+\Delta t \sigma_t}\bm{X}^{n+1,T}\bm{\widehat u}^{n}\left(\bm\Sigma -\bm{W}^{n+1}\bm{\widehat \Sigma}\bm{W}^{n+1,T} \right)\bm{W}^{n+1}\left(\bm I+\Delta t\sigma_t-\Delta t\bm{\widehat \Sigma}\right)^{-1}\\
=& (\bm S^{n} +\bm{X}^{n+1,T}\bm{\widehat u}^{n}\bm{W}^{n+1})\left(\bm I+\Delta t\sigma_t-\Delta t\bm{\widehat \Sigma}\right)^{-1}\\ 
&+ \frac{\Delta t}{1+\Delta t \sigma_t}\bm{X}^{n+1,T}\bm{\widehat u}^{n}\left(\bm I -\bm{W}^{n+1}\bm{W}^{n+1,T} \right)\bm\Sigma\bm{W}^{n+1}\left(\bm I+\Delta t\sigma_t-\Delta t\bm{\widehat \Sigma}\right)^{-1}\\
\end{align*}
Idea: Just leave out part which destroys stability. E.g. use projection of $\bm{\Sigma}$ for inscattering, i.e., use $\bm{W}^{n+1}\bm{W}^{n+1,T}\bm{\Sigma}$ instead. Hence, what we have is
\begin{align*}
    \bm S^{n+1} =& \left(\bm S^{n} + \Delta t\bm{X}^{n+1,T}\bm{\widehat u}^{n+1}\comment{\bm{W}^{n+1}\bm{W}^{n+1,T}}\bm\Sigma\bm{W}^{n+1}\right)\left(\bm I+\Delta t\sigma_t-\Delta t\bm{W}^{n+1,T}\bm\Sigma\bm{W}^{n+1}\right)^{-1},\\
\bm{\widehat u}^{n+1} =& \bm{\widehat u}^{n}(\bm I +\Delta t\sigma_t\bm I)^{-1}.
\end{align*}
So we project the solution from the previous level onto our new basis.
Now: 2-collided scheme
\begin{align*}
\bm S_{full}^{n+1}   =& \bm S^{n}\left(\bm I+\Delta t\sigma_t-\Delta t\bm{\widehat \Sigma}\right)^{-1}\\ 
&+ \Delta t\bm{X}^{n+1,T}\bm{\widehat u}^{n+1}\left(\bm\Sigma +\frac1{\Delta t}\bm I+\sigma_t\bm I -\bm{W}^{n+1}\bm{\widehat \Sigma}\bm{W}^{n+1,T} \right)\bm{W}^{n+1}\left(\bm I+\Delta t\sigma_t-\Delta t\bm{\widehat \Sigma}\right)^{-1}\\
\end{align*}

\begin{align*}
    \bm{X}^{n+1}\bm S^{n+1}\bm{W}^{n+1,T} =& \bm{X}^{n+1}\bm S^{n}\bm{W}^{n+1,T}(\bm I +\Delta t\sigma_t\bm I-\Delta t\bm\Sigma)^{-1} + \Delta t\bm{\widehat u}^{n}(\bm I +\Delta t\sigma_t\bm I)^{-1}\bm\Sigma(\bm I +\Delta t\sigma_t\bm I-\Delta t\bm\Sigma)^{-1}\\
    =& \left(\bm{X}^{n+1}\bm S^{n}\bm{W}^{n+1,T} + \Delta t\bm{\widehat u}^{n}(\bm I +\Delta t\sigma_t\bm I)^{-1}\bm\Sigma\right)(\bm I +\Delta t\sigma_t\bm I-\Delta t\bm\Sigma)^{-1}
\end{align*}

\begin{align*}
    \bm S^{n+1} = \frac1{1+\Delta t \sigma_t}\left(\bm{X}^{n+1,T}\bm{X}^{n}\bm S^{n}\bm{W}^{n}\bm{W}^{n+1,T} + \Delta t\bm{X}^{n+1,T}\bm{\widehat u}^{n+1}\bm\Sigma\bm{W}^{n+1}\right)
\end{align*}

For sake of completeness, let us state the full algorithm:
\begin{enumerate}
    \item \textbf{$K$-step streaming}: Update $\mathbf X^{n+1}\leftarrow\mathbf X^{n}$ and $\mathbf{\widetilde{S}}^n\leftarrow \mathbf{S}^n$ via
\begin{align*}
\mathbf K^{n+1} &= \mathbf L^{(1)}\mathbf K^{n} - \mathbf L^{(2)}\mathbf u(t)\mathbf{A}^T\mathbf{W}^n
\end{align*}
Determine $\mathbf X^{n+1}$ and $\mathbf{\widetilde{S}}^n$ with a QR-decomposition $\mathbf K^{n+1} = \mathbf X^{n+1} \mathbf{\widetilde{S}}^n$.
\item \textbf{$S$-step streaming}: Update $\mathbf{\widetilde{S}}^{n+1}\leftarrow\mathbf{\widetilde{S}}^{n}$ via
\begin{align*}
\mathbf{\widetilde S}^{n+1} &= \mathbf{X}^{n+1,T}\mathbf L^{(1)}\mathbf{X}^{n+1}\mathbf{\widetilde S}^{n}+\mathbf X^{n+1,T}\mathbf L^{(2)}\mathbf X^{n+1}\mathbf{\widetilde S}^{n}\mathbf W^{n,T}\mathbf{A}\mathbf W^n
\end{align*}
\item
\begin{itemize}
\item \textbf{$L$-step streaming}: Update $\mathbf L^{n+1/2}\leftarrow\mathbf L^{n}$ via
\begin{align*}
\mathbf{L}^{n+1/2} &= \mathbf{X}^{n+1,T}\mathbf L^{(1)}\mathbf{X}^{n+1}\mathbf{L}^{n}-\mathbf X^{n+1,T}\mathbf L^{(2)}\mathbf X^{n+1}\mathbf{L}^{n}\mathbf{A}^T.
\end{align*}
\item \textbf{$L$-step scattering}: Update to $\mathbf W^{n+1}$ and $\mathbf S^{n+1}$ from $\mathbf{L}^{n+1/2}$ via
\begin{align*}
\mathbf L^{n+1} =& \mathbf{L}^{n+1/2}\left(\mathbf I + \Delta t \mathbf G\right).
\end{align*}
\end{itemize}
Determine $\mathbf W^{n+1}$ and $\mathbf S^{n+1}$ with a QR-decomposition $\mathbf L^{n+1} = \mathbf W^{n+1}\mathbf S^{n+1}$.
\end{enumerate}
